''I don't want to break it'': An Exploration of Perceived Fragility in Shape-Changing Interfaces

Shape-Changing Interfaces (SCIs) dynamically alter their form, an inherent characteristic that introduces fragility into their design. As a result, users' perceptions of an interface's fragility or its potential to move or break may influence their interaction, however the extent of this effect is unclear. To address this gap, we conducted a qualitative study (N = 18) using video stimuli showcasing 20 existing SCIs. Through thematic analysis, we identified key factors impacting perceived fragility and formalized these into a framework. We then conducted a second study (N = 36) for which we fabricated SCIs that varied across selected fragility-related dimensions. We recorded user interactions and compared how the selected dimensions shaped manipulation of the objects and how they were considered by users. Together, these studies provide a structured foundational understanding of perceived fragility in SCIs and offer insights to enhance perceived robustness and inform future SCI development.

==> intro.tex <==

\section{Introduction}

Shape-changing interfaces (SCIs) are interactive systems capable of dynamically altering their physical form to provide new ways for users to interact with digital content and the physical environment \cite{alexander2018challenges, rasmussen2012shapeChangingReview}. By enabling tangible transformations such as 
bending \cite{youngwoo2015bendi}, 
rolling \cite{khalilbeigi2011xpaand}, 
expanding \cite{hirai2018xSlate, suzuki2019ShapeBots}, 
or twisting \cite{teyssier2019skinon, kim2019expandial}, 
SCIs open possibilities in areas including wearable technology, adaptive devices, robotics, and smart environments. 
They allow users to experience and manipulate interfaces through physical changes, creating richer and more engaging interaction experiences \cite{holman2008oui}.

Although SCIs promise versatility, their interactivity creates uncertainty that can amplify perceptions of fragility. Users may struggle to recognise available shape changes, hesitate to explore them, or misinterpret shape changes as unintended malfunctions (e.g. \cite{kwon2015fugaciousfilm}). Such unclear affordances may reduce confidence in the robustness of the system and reinforce concerns that experimenting with the interface might cause damage. 
These concerns are compounded by the materials and mechanisms that enable shape change. Hinges, flexible joints, soft materials, or inflatable elements are vulnerable to wear or breakage \cite{alexander2018challenges}, which can heighten user caution. 
\finalAdd{As \citeauthor{lee2023plantSci}~\cite{lee2023plantSci} note, users express \q{concern that their use of the artifacts would be damaging to the item itself, due to how they interpreted [its] form and materiality}, highlighting that fragility may \q{discourage usage}.}
Even widely adopted devices like smartphones frequently suffer breakage \cite{schaub2014broken}. What distinguishes SCIs, however, is that perceived fragility directly clashes with user expectations that novel interfaces should invite and withstand exploratory interaction.



Importantly, fragility manifests not only as a physical property but also as a \emph{user perception}, shaped by visual cues, anticipated material qualities, and expected mechanical behaviours. 
Existing studies outside the SCI domain demonstrate that perceived fragility strongly shapes user behaviour, confidence, and engagement. 
\finalChanged{For example, work on tangible objects demonstrates that physical dimensions affect fragility perception and user apprehension \cite{everitt2022investigating} while
studies involving blind users interacting with touchscreens highlight how unclear feedback can foster avoidance due to perceived fragility \cite{schaadhardt2021understanding}.}
These findings illustrate the impact of perceived fragility on interaction and highlight the importance of investigating how such perceptions influence user engagement in emerging interactive prototypes.
However, no research has directly examined how users perceive fragility in SCIs and how these perceptions affect their interactions. 
This lack of understanding limits our ability to design SCIs that are not only mechanically durable but also perceived as robust by users and subsequently invite exploration of available interactions.

To address the current lack of knowledge about perceived fragility in SCIs, we conducted a qualitative user study (N=18) where participants evaluated video stimuli showcasing 20 existing SCIs. 
Through thematic analysis of participant transcripts of a sorting task of these stimuli along a fragility spectrum, we identified 20 key factors influencing perceived fragility and formalised these into a framework. 
Building on these findings, we conducted a second study (N=36) in which we fabricated shape-changing objects that systematically varied across the selected fragility-related dimensions \emph{Material} and \emph{Demonstrated Handling} or \emph{Composition} and \emph{Movement}. 
Video recordings were analysed to examine how the selected dimensions affected interaction and perceived fragility. 
Results revealed that while some dimensions, like \emph{material} had an immediate effect on the perception of fragility, it was typically a combination of dimensions rather than isolated factors that informed participant reasoning.
Further, interaction analysis revealed that, while dimensions like \emph{movement} did not impact consciously articulated fragility perceptions, they did significantly alter behaviour patterns.

Together, these studies provide a structured foundational understanding of fragility in SCIs by revealing dimensions that inform the perception of fragility,
and exploring their impact on user behaviour.
In doing so, we offer a framework supporting the conscious consideration of fragility in the design of SCIs and subsequently encourage the development of interfaces that invite user engagement.









